Inductive Biases for Deep Learning of Higher-Level Cognition

A fascinating hypothesis is that human and animal intelligence could be explained by a few principles (rather than an encyclopedic list of heuristics). If that hypothesis was correct, we could more easily both understand our own intelligence and build intelligent machines. Just like in physics, the principles themselves would not be sufficient to predict the behavior of complex systems like brains, and substantial computation might be needed to simulate human-like intelligence. This hypothesis would suggest that studying the kind of inductive biases that humans and animals exploit could help both clarify these principles and provide inspiration for AI research and neuroscience theories. Deep learning already exploits several key inductive biases, and this work considers a larger list, focusing on those which concern mostly higher-level and sequential conscious processing. The objective of clarifying these particular principles is that they could potentially help us build AI systems benefiting from humans' abilities in terms of flexible out-of-distribution and systematic generalization, which is currently an area where a large gap exists between state-of-the-art machine learning and human intelligence.

==> conclusion.tex <==
%\Ani{Work in progress}

In this work, we have reviewed some of the many ways in which neuroscience has made fundamental contributions to advancing AI research, and argued for its increasingly important relevance. In strategizing for the future exchange between the two fields, it is important to appreciate that the past contributions of neuroscience to AI have rarely involved a simple transfer of full-fledged solutions that could be directly re-implemented in machines. Rather, neuroscience has typically been useful in a subtler way, stimulating algorithmic-level questions about facets of animal learning and intelligence of interest to AI researchers and providing initial leads toward relevant mechanisms. As such, our view is that leveraging in-sights gained from neuroscience research will expedite progress in AI research, and this will be most effective if AI re-searchers actively initiate collaborations with neuroscientists to highlight key questions that could be addressed by empirical works. Distilling intelligence into an algorithmic construct and comparing it to the human brain might yield insights into some of the deepest and the most enduring mysteries of the mind, such as the nature of creativity, dreams, and  consciousness (that's our hope).

The successful transfer of insights gained from neuroscience to the development of AI algorithms is critically dependent on the interaction between researchers working in both these fields, with insights often developing through a continual handing back and forth of ideas between fields. In the future, we hope that greater collaboration between researchers in neuro-science and AI, and the identification of a common language between the two fields, will permit a virtuous circle whereby research is accelerated through shared theoretical insights and common empirical advances. We believe that the quest to develop AI will ultimately also lead to a better understanding of our own minds and thought processes. 

The first part of the thesis was the motivated by the observation that current methods in deep learning generalize poorly to out of distribution samples. Hence,  an important challenge in machine learning is to design inductive biases and algorithms that helps the learner to generalize to out of distribution samples. We then talked about the notion of systematic generalization i.e the learner being able to generalize to samples that have zero probability under the training distribution. We note that the humans can indeed generalize in a systematic way to out of distribution samples. We then reviewed certain findings from cognitive neuroscience which may guide us in stating a set of inductive biases for achieving similar generalization in learning systems. Building upon the framework of \textit{habitual} and \textit{controlled} processing (or system 1 and system 2), where the former corresponds to habits, whereas the latter require conscious processing and attention,  we hypothesize, that an important component of system 2 processing is the decomposition of knowledge into independent pieces, that can be combined dynamically, which is also the main focus of the next chapter in this thesis. This has implications for learning deep structural models which may benefit by incorporating inductive biases which play similar role as system 2 in human brains. Till yet, deep learning as a set of principles and tools in our tool box have been very successful in solving system 1 tasks. For the coming future, the goal would be to increase tools in this toolbox by incorporating certain inductive biases to achieve similar flexibility and generalization abilities as human brains.


The second part of the thesis was based on Recurrent Independent Mechanisms \citep{RIMs}.  This work was motivated by the idea of using our understanding about the hierarchical and modular structure of the world around us in the design of neural network-based models and intelligent systems. This theme has taken us on a journey towards finding novel solutions to  object discovery, and beyond, based on a variety of neural architectures. Incorporating structure as prior knowledge takes inspiration from theories in cognitive science, such as core knowledge (Spelke and Kinzler, 2007), that posit that humans (and to some degree non-human primates) almost universally develop a number of core systems that serve as an invaluable prior (e.g., that of objectness) for understanding the structure of the world around us. Incorporating such inductive biases into neural network-based models might ultimately help us  intelligent systems that can plan, act, and achieve goals in richly structured environments and generalize in a systematic way to new and unseen circumstances.


The third part of the thesis was based on Object files and Schemta \citep{goyal2020object}.
A key goal of artificial intelligence research has been to study the dynamics of entities in the world.  We have explored the thesis that knowledge about these dynamics have a decomposition into a sparse factor graph which involves both procedural (i.e., how things act in a generic sense) knowledge and declarative knowledge (i.e., the properties of a particular entity which we have interacted with).  We proposed a concrete realization of this idea: a model that learns this decomposition dynamically using attention, into schemata (procedural) and object files (declarative).  We then found that this decomposition can be realized in many practical tasks, in which different schemata are bound for solving distinct parts of a task.  We then discussed the implications of OOP (object oritented programming) models for the symbolic/connectionist debate. OOP makes no commitment to the processing substrate in which objects are implemented. Consequently, OOP is consistent with symbolic, connectionist or even hybrid models, in which different objects within a single model are based on different computational approaches. The essential point is that each object must conform to the message-passing presuppositions (or interface requirements) of those objects with which it communicates. Thus, a further advantage of the OO approach is that it allows one to focus on the functional structure of a system while avoiding lower-level (and arguably unproductive) arguments about connectionist or symbolic processing substrate.

We've improved the inductive biases in deep learning, which along with larger scale and bigger datasets, has led to dramatically improved generalization.  While we have explored this proposal concretely, we hope to see more work in AI research think explicitly about this distinction between procedural and declarative knowledge, as well as to strengthen the link between the AI community and these widely explored concepts in cognitive psychology.  Our thesis is that this direction needs to go much further in terms of better inductive biases for higher level cognition.  We have laid out several specific ideas for pushing this forward, but we believe it is still an open field.


==> extra.tex <==
\begin{definition}[Structural Equation Model (SEM)]
    Let $\indexset_X$ be an index set. 
    An SEM $\mathcal{M}_X$ over  variables ${X = (X_i : i\in\indexset_X )}$ taking value in $\mathcal{X}$ is a triple $\left(\mathcal{S}_X, \mathcal{I}_X, \mathbb{P}_{E} \right)$ where
    \vspace{-.5em}
    \begin{itemize}[noitemsep]
        \item $\mathcal{S}_X$ is a set of structural equations, i.\,e.\ it is a set of equations $X_i = f_i\left( X , E_i \right)\ $ for $i \in \indexset_X$;
        \item ($\mathcal{I}_X, \leq_X)$ is a subset of all perfect interventions equipped with a natural partial ordering (see below), i.\,e.\ it is an index set where each index corresponds to a particular perfect intervention on some of the $X$ variables;
        \item $\mathbb{P}_{E}$ is a distribution over the exogenous variables $E = ( E_i : i\in\indexset_X)$;
        \item with $\mathbb{P}_E$-probability one, under any intervention ${i \in \mathcal{I}_X}$ there is a unique solution $x\in\mathcal{X}$ to the intervened structural equations. This ensures that for any intervention ${i \in \mathcal{I}_X}$, $\mathcal{M}_X$ induces a well-defined distribution over $\mathcal{X}$.%
\footnote{That is, with probability one over the exogenous variables $E$, for each draw $E=e$ there exists a unique value $x\in \mathcal{X}$ such that $e$ and $x$ satisfy the intervened structural equations. The distribution of $E$ in conjunction with $\mathcal{S}_X$ then implies a distribution over $\mathcal{X}$ for each intervention $i \in \mathcal{I}_X$ via these unique solutions.
If the SEM is acyclic, this is always satisfied.}
    \end{itemize}
    \vspace{-.5em}
\end{definition}

In an SEM, each $X_i$ is a function of the $X$-variables and the exogenous variable $E_i$.
In this mathematical model, a perfect intervention on a single variable $\doop(X_i=x_i)$ is realised by replacing the structural equation for variable $X_i$ in $\mathcal{S}_X$ with $X_i = x_i$.
Perfect interventions on multiple variables, e.g. $\doop(X_i=x_i, X_j=x_j)$, are similarly realised by replacing the structural equations for each variable individually.
Elements of $\mathcal{I}_X$ correspond to perfectly intervening on a subset of the $X$ variables, setting them to some particular combination of values.

$\mathcal{I}_X$ has a natural partial ordering in which, for interventions ${i, j \in \mathcal{I}_X}$, ${i\leq_X j}$ if and only if $i$ intervenes on a subset of the variables that $j$ intervenes on and sets them equal to the same values as $j$. 
For example, ${\doop(X_i=x_i) \leq_X \doop(X_i=x_i, X_j=x_j)}$.\footnote{Informally, this means that $j$ can be performed after $i$ without having to change or undo any of the changes to the structural equations made by $i$. 
Not all pairs of elements must be comparable: for instance, if $i= \doop(X_1=x_1)$ and $j = \doop(X_2=x_2)$, then neither $i\leq_X j$ nor $j \leq_X i$.} 

The purpose of the following example is to illustrate how SEMs are written in our notation and to provide and example of a restricted set of interventions $\mathcal{I}_X$.

\begin{example}\label{example1}
Consider the following SEM defined over the variables $\{ B_1,B_2,L \}$
%
\begin{align*}
\mathcal{S}_X = \big\{ & B_1 = E_1,\ B_2 = E_2,\ L = \operatorname{OR}(B_1,B_2,E_3) \big\} \\
%
\mathcal{I}_X = \big\{ & \nulli,\ \doop(B_1=0),\ \doop(B_2=0),\\
& \doop(B_1=0,B_2=0) \big\}, \\
%
\{ E_1,E_2,E_3 \} & \overset{\text{iid}}{\sim} \mathrm{Bernoulli}(0.5)
\end{align*}
%
where by the element $\nulli \in \mathcal{I}$ we denote the null-intervention corresponding to the unintervened SEM\@.
\end{example}

\section{SEMs for Causal Modelling}\label{sec:sem-for-causal-modelling}

In addition to being abstract mathematical objects, SEMs are used in causal modelling to describe distributions of variables and how they change under interventions \citep{}.
The $\doop$-interventions as abstract manipulations of SEMs are understood as corresponding to actual (or potentially only hypothetical) physical implementations in the real world, i.\,e.\ the model is `rooted in reality'.
For instance, if a binary variable $B_1$ in an SEM reflects whether a light bulb is emitting light, then $\doop(B_1=0)$ could be achieved by flipping the light switch or by removing the light bulb.

The SEM in Example~\ref{example1} could be thought of as a simple causal model of two light bulbs $B_1$ and $B_2$ and the presence of light $L$ in a room with a window.
Suppose that we have no access to the light switch and there are no curtains in the room but that we can intervene by removing the light bulbs.
We can model this restricted set of interventions by $\mathcal{I}_X$, i.\,e.\ the $\doop$-intervention on the SEM side ${\doop(B_1=0)}$  corresponds to removing the light bulb $B_1$.

The partial ordering of $\mathcal{I}_X$ corresponds to the ability to compose physical implementations of interventions. The fact that we can first remove light bulb $B_1$ (${\doop(B_1=0)}$) and then afterwards remove light bulb $B_2$ (resulting in the combined intervention ${\doop(B_1=0, B_2=0)}$)  is reflected in the partial ordering via the relation ${\doop(B_1=0) \leq_X \doop(B_1=0,B_2=0)}$.
%
